Computational micromagnetics with Commics

We present our open-source Python module Commics for the study of the magnetization dynamics in ferromagnetic materials via micromagnetic simulations. It implements state-of-the-art unconditionally convergent finite element methods for the numerical integration of the Landau-Lifshitz-Gilbert equation. The implementation is based on the multiphysics finite element software Netgen/NGSolve. The simulation scripts are written in Python, which leads to very readable code and direct access to extensive post-processing. Together with documentation and example scripts, the code is freely available on GitLab.

==> pgflibrarypgfplots.colorbrewer.code.tex <==
\usetikzlibrary{colorbrewer}
\pgfplotscreateplotcyclelist{mBlueToRed}{%
  mBlueToRed-1\\%
  mBlueToRed-2\\%
  mBlueToRed-3\\%
  mBlueToRed-4\\%
  mBlueToRed-5\\%
  mBlueToRed-6\\%
}
\pgfplotsset{
colormap={mBlueToRed}{
  color=(mBlueToRed-1);
  color=(mBlueToRed-2);
  color=(mBlueToRed-3);
  color=(mBlueToRed-4);
  color=(mBlueToRed-5);
  color=(mBlueToRed-6);
}
}


==> tikzlibrarycolorbrewer.code.tex <==
\definecolor{mBlueToRed-1}{RGB}{33,102,172}
\definecolor{mBlueToRed-2}{RGB}{103,169,207}
\definecolor{mBlueToRed-3}{RGB}{209,229,240}
\definecolor{mBlueToRed-4}{RGB}{253,219,199}
\definecolor{mBlueToRed-5}{RGB}{239,138,98}
\definecolor{mBlueToRed-6}{RGB}{178,24,43}

